Semileptonic $B \to D^{(\ast)} \ell\nu$ Decay Form Factors using the Oktay-Kronfeld Action

We report recent progress in calculating semileptonic form factors for the $\bar{B} \to D^\ast \ell \bar{\nu}$ and $\bar{B} \to D \ell \bar{\nu}$ decays using the Oktay-Kronfeld (OK) action for bottom and charm quarks. We use the second order in heavy quark effective power counting $\mathcal{O}(\lambda^2)$ improved currents in this work. The HISQ action is used for the light spectator quarks. We analyzed four $2+1+1$-flavor MILC HISQ ensembles with $a\approx 0.09\,\mathrm{fm}$, $0.12\,\mathrm{fm}$ and $M_\pi \approx 220\,\mathrm{MeV}$, $310\,\mathrm{MeV}$: $a09m220$, $a09m310$, $a12m220$, $a12m310$. Preliminary results for $B\to D^\ast\ell\nu$ decays form factor $h_{A_1}(w)$ at zero recoil ($w=1$) are reported. Preliminary results for $B \to D\,\ell\nu$ decays form factors $h_\pm(w)$ over a kinematic range $1<w<1.3$ are reported as well.

==> table/tab_kappa.tex <==
%\vspace{-2em}

\begin{table}[h!]
\centering
  \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{@{\quad}c @{\quad}|@{\quad}c@{\quad}|@{\quad}c@{\quad}|@{\quad}c@{\quad}|@{\quad}c@{\quad}|@{\quad}c@{\quad}|@{\quad} c @{\quad}}
      \hline\hline
      ID & $\kappa_\text{crit}$ & $\kappa_c$ & $\kappa_b$ & $\{\sigma,N\}$ & $N_\text{cfg} \times N_\text{src}$ & $\tau$ \\
      \hline
      a12m310 & 0.051211 & 0.048524 & 0.04102 & \{1.5,\,5\} & $1053 \times 3$ & 10, 11, 12, 13, 14, 15\\
      a12m220 & 0.051218 & 0.048613 & 0.04070 & \{1.5,\,5\} & $1000 \times 3$ & 10, 11, 12, 13\\
      \hline
      a09m310 & 0.05075 & 0.04894 & 0.0429 & \{2,\,10\} & $1001 \times 3$ & 15, 16, 17, 18\\
      a09m220 & 0.05077 & 0.04902 & 0.0431 & \{2,\,10\} & $1001 \times 3$ & 15, 16, 17, 18\\
      \hline\hline
  \end{tabular}}
  \caption{The hopping parameters for bottom and charm valence quarks
    and the CGS parameters. Here, $N_\text{cfg}$ represents the number
    of gauge configurations used for measurement. $N_\text{src}$
    represents the number of sources used for measurement per gauge
    configuration.}
  \label{tab:kappa}
\end{table}

